vCLIC: Towards Fast Interrupt Handling in Virtualized RISC-V Mixed-criticality Systems

The widespread diffusion of compute-intensive edge-AI workloads and the stringent demands of modern autonomous systems require advanced heterogeneous embedded architectures. Such architectures must support high-performance and reliable execution of parallel tasks with different levels of criticality. Hardware-assisted virtualization is crucial for isolating applications concurrently executing these tasks under real-time constraints, but interrupt virtualization poses challenges in ensuring transparency to virtual guests while maintaining real-time system features, such as interrupt vectoring, nesting, and tail-chaining. Despite its rapid advancement to address virtualization needs for mixed-criticality systems, the RISC-V ecosystem still lacks interrupt controllers with integrated virtualization and real-time features, currently relying on non-deterministic, bus-mediated message-signaled interrupts (MSIs) for virtualization. To overcome this limitation, we present the design, implementation, and in-system assessment of vCLIC, a virtualization extension to the RISC-V CLIC fast interrupt controller. Our approach achieves 20x interrupt latency speed-up over the software emulation required for handling non-virtualization-aware systems, reduces response latency by 15% compared to existing MSI-based approaches, and is free from interference from the system bus, at an area cost of just 8kGE when synthesized in an advanced 16nm FinFet technology.

==> tab/rel_work.tex <==
\begin{table*}[t]
    \caption{Comparison of the main interrupt virtualization techniques in industrial and research computing architectures.}
    \begin{center}
    \setlength{\tabcolsep}{1.5pt} % Tune column width
    \renewcommand{\arraystretch}{1.3} % Tune row height (vertical spacing)
    \resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{lccccccccc}

    \multirow{2}{*}{\rotatebox{0}{\textbf{Reference}}} &
    \multirow{2}{*}{\rotatebox{0}{\textbf{ISA}}} & 
    \multirow{2}{*}{\rotatebox{0}{\textbf{\thead{Virtualization \\ technology}}}} & 
    \multirow{2}{*}{\rotatebox{0}{\textbf{\thead{Interrupt \\ controller}}}} & 
    \multirow{2}{*}{\rotatebox{0}{\textbf{\thead{Interrupt \\ type}}}} & 
    \multirow{2}{*}{\rotatebox{0}{\textbf{Open?}}} & 
    \multirow{2}{*}{\rotatebox{0}{\textbf{\thead{Application target}}}} &
    \multicolumn{3}{c}{\rotatebox{0}{\textbf{Real time features}}} \\
        \cline{8-10}
        & & & & & & & \textbf{Selective-vectoring} & \textbf{Nesting} & \textbf{Tail-chaining} \\
        \hline
    
    \hline 
    
     Intel & Intel x86-64, IA-32 & Intel VT-x  & APICv     & \gls{msi} / wired & \xmark & High-performance / GP computing & \xmark & \xmark & \xmark \\
    
    AMD & AMD x86-64             & AMD-V       & AVIC      & \gls{msi} / wired & \xmark & High-performance / GP computing & \xmark & \xmark & \xmark \\
    
    ARM Cortex-A & Aarch64    & ARMv7/8-A     & GICv2/3/4     & \gls{msi} / wired              & \xmark & Embedded, application-class & \xmark & \xmark & \xmark \\
    
    % ARM Cortex-A & Aarch64    & ARMv8-A     & GICv3/4   & \gls{msi}              & \xmark & Embedded, application-class & \xmark & \xmark & \xmark \\

    ARM Cortex-R & Aarch32/64 & ARMv8-R & GICv3/4 & \gls{msi} / wired & \xmark & Real-time, application-class & \xmark & \xmark & \xmark \\

    ARM Cortex-M & Aarch32    &       -     & NVIC      & wired              & \xmark & Embedded, real-time & \cmark & \cmark & \cmark \\
    
    RISC-V & RV64GCH          & H-extension & AIA       & \gls{msi}              & \cmark & High-performance / GP computing & \xmark & \xmark & \xmark \\ 
    
    \hline
    
     S{a}'~et~al.~\cite{VPLIC}&  RV64GCH          & H-extension & vPLIC     & Wired                  & \cmark & Embedded, \gls{mcs} & \xmark & \xmark & \xmark \\
    
    Marques~et~al.~\cite{IEAIA_MINHO } & RV64GCH          & H-extension & IE-AIA    & MSI              & \cmark & Embedded, \gls{mcs} & \xmark & \xmark & \xmark \\
    
    \textbf{This work} & \textbf{RV64GCH}          & \textbf{H-extension} & \textbf{vCLIC}     & \textbf{Wired}                  & \cmark & \textbf{Embedded}, \textbf{\gls{mcs}} & \cmark & \cmark & \cmark \\
    

    % for Renesas: IPL is 3 bits wide and indicates the Interrupt Priority Level (IPL) from level 0 to level 7. If a requested interrupt has higher priority level than IPL, the interrupt is acknowledged.

    % \hline 
    % \multicolumn{7}{l}{\textbf{Academia}} \\ 
    % \hline 
    
    % Gaitan et al.~\cite{TASK_SWITCHING_TVLSI} & MPRA/HSE & RISC & Automatic in \gls{hw} & Automatic in \gls{hw} & n.a. & \xmark & n.a. & 1.5~\tnote{d} & 3~\tnote{d} & n.a. \\
    % Mao et al.~\cite{mao_2021} & CLIC & RISC-V & Automatic in \gls{hw} & n.a. & n.a.~\tnote{e} & \xmark & n.a. & 13 & n.a. & \rebuttal{\SI{4}{\kilo GE}}~\tnote{h} \\
    % \rebuttal{Huang et al.~\cite{paged_regfile}} & \rebuttal{n.a.} & \rebuttal{Arm RISC} & \rebuttal{-} & \rebuttal{valid-annotated mechanism and semi-shadowing} & \rebuttal{-} & \rebuttal{\cmark} & \rebuttal{n.a.} & \rebuttal{n.a.} & \rebuttal{n.a.} & \rebuttal{n.a.} \\
    % Balas et al.~\cite{balas_2021} & CLINT & RISC-V & - & - & - & \cmark & - & 24 & 129 & \rebuttal{\SI{10}{\kilo GE}} \\
    % \textbf{This work} & \textbf{CLIC} & \textbf{RISC-V} & \textbf{Hybrid}~\tnote{\textbf{f}} & \textbf{Hybrid} & \texttt{\textbf{emret}} & \cmark & \textbf{256} & \textbf{6} & \textbf{114} & n.a. \\
    \hline   
    \end{tabular}
    % \begin{tablenotes}
    % \item[a] Single high-speed interrupt. Refers to the number of clock cycles from the firing of an interrupt to the execution of the interrupt body. Does not count the saving of the general purpose registers.~\cite{renesas_m32c80}.
    % \item[b] Refers to the number of cycles from arrival the arrival of the interrupt to the first instruction fetch of the \gls{isr}~\cite{sifive_e21}. Does not count the saving of the interrupt context, including the general purpose registers.
    % \item[c] Refers to the number of the clock cycles it takes from the firing of an external interrupt to the time the first instruction in the corresponding interrupt service routine of a C function is executed~\cite{nuclei_isa}.
    % \item[d] Full \gls{hw} solution. \Gls{sw} scheduling latency becomes negligible as from~\cref{fig:int-latency-decomposed}, which justifies the performances in the order of the clock cycle.
    % \item[e] Implementation details are omitted.
    % \item[f] Combination of background saving/restoring and register banking.
    % \item[g] \rebuttal{Commercial architectures do not report overheads and costs.}
    % \item[h] \rebuttal{Implemented in a 0.11$\mu$m technology node. Total size of the interrupt system.}
    % \end{tablenotes}
    \end{threeparttable}
    }
    
    \label{tab:related_work}
    \end{center}
\end{table*}


==> text/Background.tex <==
\section{Background}
\label{sec:back}

\begin{figure}[t]
    \centering
    %\includesvg[width=0.9\columnwidth]{fig/privilege_modes.svg}
    \includegraphics[width=0.9\columnwidth]{fig/privilege_levels.pdf}
    % \setlength{\belowcaptionskip}{-25pt}
    \caption{RISC-V privilege modes according to H-extension.}
    \label{fig:riscvh}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{fig/cheshire.pdf}
%     \caption{The Cheshire platform. {\vclic} and interrupt subsystem are highlighted.}
%     \label{fig:cheshire}
% \end{figure}

\begin{figure}[t]
    \centering
    % \begin{subfigure}{\textwidth}
    %     \includegraphics[width=\columnwidth]{fig/cheshire.pdf}
    %     \label{fig:cheshire:system}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{\textwidth}
    %     \includesvg[width=\columnwidth]{fig/CLIC-CVA6.svg}
    %     \label{fig:cheshire:zoomin}
    % \end{subfigure}
    \subfloat[Cheshire platform diagram. Per-core vCLIC is highlighted.]{\label{fig:cheshire:system}\includegraphics[width=\columnwidth]{fig/cheshire.pdf}}\\
    \subfloat[CLIC and CVA6 interface. Only relevant parts of the core are shown.]{\label{fig:cheshire:zoomin}\includegraphics[width=\columnwidth]{fig/vCLIC-CVA6.pdf}}%
    \vspace{.1cm}
    \caption{Cheshire (a) and its interrupt subsystem (b).}
    \label{fig:cheshire}
\end{figure}

\subsection{Virtualization Technology}\label{subsec:back:vt}

Virtualization enables the creation of virtual hardware, operating systems, applications, or networks within a single physical computing system. It decouples \gls{sw} and services from the underlying \gls{hw}, allowing multiple independent environments to execute concurrently and in isolation. This capability is crucial in modern \glspl{mcs}, where minimizing interference among safety- and time-critical software components is essential to meet stringent real-time requirements~\cite{AUTOMOTIVE_PREDICTABLE}.

\subsubsection{Virtual Machine (Guest)}\label{subsubsec:back:vt:vm}
A Virtual Machine (\gls{vm}) is a software emulation of a physical computer, including its processor, memory, storage, and networking interfaces. Multiple \glspl{vm} can coexist on a single physical machine, each operating its own guest \gls{os} and applications. \glspl{vm} ensure a high degree of isolation, allowing efficient resource utilization and workload management.

\subsubsection{Virtual Machine Monitor (Hypervisor)}\label{subsubsec:back:vt:vmm}
A \gls{vmm}, or hypervisor, is a software layer positioned between the \gls{hw} and the \glspl{vm}. It manages and allocates physical resources among various \glspl{vm}, ensuring they operate independently and securely.

\subsubsection{HW-assisted Virtualization in RISC-V}\label{subsubsec:back:vt:hwvirtriscv}
Under the \mbox{RISC-V} privileged architecture specification~\cite{RISCV_II}, \gls{hw}-assisted virtualization is enabled through the hypervisor \texttt{H} extension. This extension elevates the supervisor mode to the hypervisor-extended supervisor mode (\texttt{HS}). HS-mode operates similarly to S-mode but includes additional instructions and \glspl{csr} for hosting a guest \gls{os} in \gls{vs} mode. Regular S-mode \glspl{os} can run unchanged either in \gls{hs}-mode or as \gls{vs}-mode guests. 
\Cref{fig:riscvh} illustrates RISC-V's privilege mode stack when the \texttt{H} extension is enabled.

\subsection{Static and Dynamic Partitioning Hypervisor}\label{subsec:back:spdh}
\Glspl{sph} help platforms meet the rigorous demands of industry safety standards like \texttt{IEC61508} by pinning specific system resources to a single \gls{vm} without an intermediate scheduler. The hypervisor and \gls{vm} resources are statically allocated and mapped during the system's boot or initialization phase~\cite{SPH_MINHO}.

Conversely, \glspl{dph} allow flexible allocation of processor cores and memory usage, enabling multiple \gls{vm} guests to share the same physical resources. Such a setting is more challenging for embedded \glspl{mcs} as guests share resources with potentially different criticality levels and hence priority. 
%From an interrupt management perspective, we address this issue with the VSPRIO extension in {\vclic} (\cref{subsubsec:arch:vsprio}).

\subsection{Interrupt Terminology}\label{subsec:back:term}

\subsubsection{Types}\label{subsubsec:back:term:intrs}

Interrupts are asynchronous events that disrupt the normal order of program execution, necessitating a context switch to an \textit{interrupt context} -- a process known as \textit{preemption}. \textit{Vectored} interrupts have dedicated \glspl{isr} which the core can directly call. This mode of operation enables quick responses, which are crucial for real-time systems.
In contrast, \textit{non-vectored}, or \textit{direct}, interrupts use a shared \gls{isr} within which additional instructions are required to determine the source of the interrupt.
Interrupts initiated from different privilege modes are referred to as \textit{vertical}, while those from the same privilege mode are \textit{horizontal}.

\subsubsection{Interrupt Latency}\label{subsubsec:back:term:lat}

%This paper focuses on minimizing the \gls{hw}-imposed latency of interrupts. 
\textit{Interrupt latency} is the time from an interrupt signal reaching the hardware, typically an interrupt controller, to the start of execution of the \gls{isr}'s first instruction. This first instruction follows saving all necessary context on the stack, enabling the subsequent function call, as dictated by the \gls{isa}'s calling convention. For time-critical tasks, which usually follow a real-time periodic model~\cite{buttazzo2011hard}, it is essential to minimize and stabilize interrupt latency and jitter over multiple periods.

\subsubsection{Interrupt Jitter}\label{subsubsec:back:term:jit}
Modern embedded \glspl{mcs} rely on application-class cores with increasingly complex architectures to sustain the growing software stack and computational requirements of application domains such as automotive, aerospace, or humanoid robotics. 
Consequently, the interrupt response time (i.e., its absolute value and variability over time) of these architectures is highly affected by the micro-architectural state of the system. 
An in-depth analysis of such effects is required in order to assess the worst-case behavior of hard real-time constrained \gls{mcs}. 
% This is especially true for cached memory accesses, such as fetching instructions for an \gls{isr} or performing a page-table walk upon a page-fault exception, where a cache miss can cause delays ranging from tens to hundreds of clock cycles. 
% These features complicate real-time analysis and hinder a predictable behavior.

\subsection{RISC-V CLIC and real-time features}\label{subsec:back:clic}

The RISC-V \texttt{smclic} specification~\cite{clic} outlines the operation of a fast interrupt controller suitable for \texttt{M} and \texttt{S} privilege modes in the embedded domain. It supports prioritization of interrupts through \textit{levels} and \textit{priorities}.
% Interrupts are managed based on a \textit{threshold value} set through a \gls{csr}, facilitating interrupt nesting. 
Interrupt nesting is controlled by a \textit{threshold value} stored in a \gls{csr}, allowing higher-level incoming interrupts to preempt the current execution.
The \gls{shv} feature allows to configure interrupts as vectored or non-vectored during runtime. Additionally, the \texttt{xnxti} extension enhances the handling of consecutive interrupts through efficient redundant context restoration, a technique also known as tail-chaining. These capabilities render the \gls{clic} an optimal solution for rapid real-time interrupt management in RISC-V systems.


==> text/Related_Work.tex <==
\section{Related Work}
\label{sec:relwork}

\input{tab/rel_work}

%Over the years, all the major computing architectures have evolved to support virtualization in hardware. 
Adopting virtualization in real-time embedded systems has raised the need for \gls{hw} support in interrupt controllers to enable fast responsiveness to time-critical events in virtualized systems~\cite{HEISER_VIRT}. 
\Cref{tab:related_work} provides an overview of the main virtualization techniques for interrupt controllers in industry and academia and compares real-time and predictability features against our work. 
We identify three main characteristics of an interrupt controller tuned for fast interrupt handling: selective vectoring, interrupt nesting, and tail-chaining (\cref{subsec:back:clic}).

% Intel / AMD section

Since the 12th generation of the Intel Core processor, the Intel Virtualization Technology (Intel VT-x) \cite{intel_64_manual} has been extended to support interrupt virtualization. The Intel APIC Virtualization Technology (Intel APICv) adds virtualization features to the Advanced Programmable Interrupt Controller (APIC), allowing delivery of interrupts to virtual machines and \gls{hw} emulations of APIC accesses.
AMD has followed this trend by integrating the AMD AVIC into its AMD-V virtualization technology. However, these architectures target general-purpose high-performance computing systems, lacking support for the real-time and predictable market segment. 

% Arm section

% Arm Cortex-A family and GICv2/3/4
On the other end of the spectrum, RISC architectures have dominated the real-time and embedded processing domains. Arm introduced hardware virtualization support in its Armv7-A application class architecture. Arm cores belonging to the Cortex-A family manage interrupts using the platform-level (centralized) Generic Interrupt Controller (GIC). Support for interrupt virtualization was first introduced in GICv2 and further extended in the latter GICv3 and GICv4 interrupt controllers, supported by the latest family of Arm application class cores, Armv8-A. 
Hardware support for direct injection of interrupts to \glspl{vm} was only introduced with GICv4. This eliminated the need for hypervisor intervention for interrupts directed to currently executing \glspl{vm}. Nevertheless, this implementation required context switching the GIC virtual interrupt registers when changing the scheduled processing resource, affecting the worst-case interrupt latency.
% Until GICv3, interrupt virtualization required the intervention of privileged software: physical interrupts are signaled to a hypervisor, which can then generate virtual interrupts by writing a virtualization control register file. Moreover, this implementation required context switching the GIC virtual interrupt registers when changing the scheduled processing resource.
% Finally, GICv4 introduced support for hypervisor-agnostic virtual interrupt injection.
%, reducing virtual interrupt latency.
%by eliminating the need for hypervisor intervention. 

% Arm Cortex-M family and NVIC
Nevertheless, the GIC interrupt controller is not designed to minimize the interrupt latency and lacks features such as vectoring and tail-chaining. Arm supports fast interrupt response through the core-local Nested Vectored Interrupt Controller (NVIC), used in microcontrollers based on the Arm Cortex-M processor family, targeting low-power embedded systems. However, the NVIC is not designed with virtualization in mind.
% and does not provide any of the virtualization features of the GIC.

% Arm Cortex-R family
Finally, processors belonging to the Arm Cortex-R family, such as the \SI{32}{\bit} Cortex-R7 and the \SI{64}{\bit} Cortex-R82 cores, designed for high-performance time- and safety-critical applications, also inherited part of the virtualization support introduced by the Armv7-A architecture. Since they also rely on the GIC interrupt controller, such processors have the same limitations as the Cortex-A family concerning fast interrupt processing. 

% On the other end of the spectrum, RISC architectures have dominated the real-time and embedded processing domains. Arm has supported virtualization since the ARM-v7-A application class architecture and interrupt virtualization since GICv2. The next generation of ARM application class cores (Armv8-A) includes GICv3 and GICv4, which extend virtualization support. 
% In GICv3, a set of dedicated configuration registers is exposed to the vPE (virtual Processing Engine) running on the core. Interrupts are signaled to the hypervisor at the physical level, which injects them into vPEs by setting a dedicated interrupt pending register in the interrupt controller. During a vPE context switch, the hypervisor must save the virtual interrupt configuration registers of the GIC, impacting worst-case interrupt latency.

% Since GICv4's release, ARM has added support for direct injection of virtual interrupts. However, the support for virtual interrupt injection is limited to \glspl{msi}, that are generated by peripherals or by \gls{sw}. Despite providing extensive support for interrupt virtualization, the ARM GIC interrupt controller has been designed for the application class category of ARM cores, and do not have support for real-time processing. 

% On the other hand, the ARM Nested Vectored Interrupt Controller (NVIC) is typically used in ARM Cortex-M-based microcontrollers, which are designed for low-power, real-time applications and embedded systems. Nevertheless, the NVIC is not designed with virtualization in mind, and does not provide any of the virtualization features of the GIC.

% \todo{TODO1: add Arm FIQ as an example of critical interrupt support}

% RISC-V section

Within the RISC-V ecosystem, S{a}~et~al.~\cite{VPLIC} enhanced the RISC-V Platform Level Interrupt Controller (PLIC) to support interrupt virtualization with a custom extension. While significantly improving the best-case interrupt latency over alternative software emulation approaches, the PLIC does not support any of the aforementioned real-time features but has the advantage of being a centralized design, reducing overall area overhead. 
% which lacks real-time interrupt response features. 
The RISC-V \gls{aia} was recently ratified to replace the original RISC-V interrupt subsystem~\cite{aia}. AIA supports interrupt virtualization using \glspl{msi} by means of: (i) the Advanced PLIC (A-PLIC), which extends the PLIC to generate \glspl{msi} via the system bus, and (ii) the \gls{imsic}, a core-local controller that receives \glspl{msi} and interfaces with a RISC-V core.

Akin to other ISAs reported in~\cref{tab:related_work}, AIA is designed for high-performance computing systems and lacks key real-time features found in RISC-V \gls{clic} or ARM's NVIC. \glspl{msi} typically transmit over the system bus, reducing predictability and worsening interrupt latencies during bus contention. To address this issue, Marques~et~al.~\cite{IEAIA_MINHO} proposed the Integrated-Embedded AIA (IE-AIA) for real-time mixed-criticality embedded systems, using a single IMSIC instance shared among up to four cores, coupled with a platform-level A-PLIC. 
This design mitigates bus interference effects typical of \gls{msi}-based systems. Although improving predictability of virtual \glspl{msi}, IE-AIA still lacks support for real-time fast-interrupt response. 
%As detailed in~\cref{subsec:eval:func}, our {\vclic} implementation provides improved interrupt latency in isolation by approximately \SI{15}{\percent}.

% Enrico
% I believe the flow could be: 
% - 1/2 sentences of overview that motivate interrupt virtualization. 
% - Intel/AMD virtualization technlogy as a reference of widespread computing architectures (but not targeting embedded real-time)
% - Move to efficient RISC architectures and present ARM's virtualization extension and support for interrupt virtualization in GIC.
% - Move to RISC-V as open-source ISA leader and mention efforts to extend virtualization support. 
% - Mention vPLIC from Minho.
% - Discuss AIA and its limitations
% - Conclude AIA comparison by listing nice features of CLIC for real-time

%Important for context; from RISC-V AIA spec:
%This initial version of the Advanced Interrupt Architecture is focused primarily on the needs of larger, high-performance RISC-V systems. Support is not currently defined for the following interrupt-handling features that are useful for minimizing interrupt response times in so-called “real-time” systems but are less appropriate for high-speed processor cores: 
%* the option to give each interrupt source at a hart a separate trap entry address;
%* automatic stacking of register values on interrupt trap entry, and restoration on exit; and
%* automatic preemption (nesting) of interrupts at a hart, based on priority.
%It is intended that such features optimizing for smaller and/or real-time systems can be developed as a follow-on extension, either separately or as part of a future version of the interrupt architecture of this document.



==> text/archi_2.tex <==
\section{Architecture}
\label{sec:arch}

In virtualized RISC-V systems, the {\vclic} extension allows a hypervisor to delegate individual interrupts to \glspl*{vm}. The delegation reduces interrupt latency by eliminating the hypervisor-mediated \gls*{sw} emulation of the \gls*{ic}. The {\vclic} is integrated into the Cheshire platform~\cite{10163410}, briefly described in~\cref{subsec:arch:cheshire}. The {\vclic} design is split into two modular extensions: (i) \texttt{VSCLIC}, which enables the delegation of interrupt lines to \glspl*{vm}, and (ii) \texttt{VSPRIO}, which allows the hypervisor to prioritize interrupts depending on the \gls*{vm} they are assigned to, as discussed in~\cref{subsec:arch:vclic}. Furthermore, the enhancements required in the core (in this work, CVA6) connected to the {\vclic} are described in~\cref{subsec:arch:cva6}. \Cref{fig:cheshire} details the {\vclic}-CVA6 interface, highlighting the novel \gls*{hw} features compared to vanilla \gls*{clic}.

\subsection{Cheshire Platform}\label{subsec:arch:cheshire}

Cheshire~\cite{10163410} is a minimal system built around the 64-bit, application-class CVA6 RISC-V processor~\cite{CVA6}. The platform is highly configurable, supporting seamless integration of domain-specific accelerators or other general-purpose engines with diverse criticality levels via an AXI4 fully connected crossbar, as shown in \cref{fig:cheshire}. 
%\Cref{fig:cheshire} illustrates Cheshire's high-level block diagram. 
%It shows how incoming interrupts from peripheral devices are masked and distributed to each core via a programmable interrupt router and then locally managed by the corresponding {\vclic}.
In a multi-core setup, each {\vclic} instance is tightly coupled to each core, ensuring independence from the system bus and thereby eliminating interference at the interconnect level. % --- a critical feature in \glspl*{mcs}, where shared resources often become performance bottlenecks and complicate real-time analysis~\cite{benz2023axirealm}.

\subsection{{\vclic} extension}\label{subsec:arch:vclic}

% \vspace{0.1cm}

\subsubsection{VSCLIC}\label{subsubsec:arch:vsclic}

The \texttt{VSCLIC} extension allows to delegate interrupt lines to \gls*{vs} mode. It introduces a new set of memory-mapped configuration registers, namely \texttt{clicintv}, that are under the control of the hypervisor (\cref{fig:cheshire}). For each interrupt line \emph{i}, \texttt{clicintv[\emph{i}]} is a \SI{1}{\byte} register comprising (i) a virtualization bit (\emph{v} field), which adds a new orthogonal privilege mode to the privilege mode interrupt attribute, and (ii) a virtual supervisor ID (\emph{vsid} field), which holds the \gls*{vsid} of the \gls*{vm} to which the interrupt is delegated.

%Since each interrupt line can only be assigned to one \emph{interrupt target} (i.e. a software component identified by privilege mode or guest ID) at a time, the 
{\vclic} multiplexes the virtual configuration registers of each target on a single set of physical registers, minimizing the area overhead on the register file. 
%The configuration of interrupt lines delegated to higher-privilege modes appears to be hardwired to zero to lower-privileged software. 
The privilege of software accessing {\vclic} configuration registers is determined by the address range used to access them by partitioning the {\vclic} configuration address space. To guarantee isolation, each \gls*{vm} must be granted access to only one of these address regions (i.e., the one associated with its \gls*{vsid}). Such isolation can be enforced by privileged software by means of \gls*{pmp} units or --- on systems supporting two-stage address translation --- by virtual memory.
 
% \vspace{0.1cm}

\subsubsection{VSPRIO}\label{subsubsec:arch:vsprio}

The {\vclic} supports up to 64 simultaneous active guests, identified by a \gls*{vsid} stored in the \emph{VGEIN} field of the \emph{hstatus} \gls*{csr}, as per the \mbox{RISC-V} \texttt{H} extension. This allows to statically delegate interrupt lines of pass-through peripherals to \glspl*{vm}, eliminating the need of saving and restoring the \gls*{ic} configuration upon \gls*{vm} context switch, thereby improving the worst-case interrupt latency. 

Nevertheless, to ensure that the real-time properties of interrupts delegated to safety-critical guests are not affected, the \texttt{VSPRIO} extension allows the hypervisor to prioritize virtual interrupts based on the associated \glspl*{vm}. The extension enlarges the interrupt priority space by adding a set of privileged configuration registers that hold a per-\gls*{vm} priority value. This enables dynamic prioritization of real-time and safety-critical \glspl*{vm}, allowing the deployment of systems with more tightly bound worst-case interrupt latencies. 

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.9\columnwidth]{example-image-b}
%     % \includegraphics[width=\columnwidth]{fig/cheshire.png}
%     \includegraphics[width=\columnwidth]{fig/vclic_cva6.png}
%     % \includesvg[width=\columnwidth]{fig/vclic_cva6_helv.svg}
%     \caption{Cheshire (a) and its interrupt subsystem (b).}
%     \label{fig:cheshire}
% \end{figure}

\begin{figure}[t]
    \centering
    \subfloat[Cheshire platform diagram. Per-core vCLIC is highlighted.]{\label{fig:cheshire:system}\includegraphics[width=0.95\columnwidth]{fig/cheshire.png}}\\
    \subfloat[CLIC and CVA6 interface. Only relevant parts of the core are shown.]{\label{fig:cheshire:zoomin}\includegraphics[width=0.95\columnwidth]{fig/vclic_cva6.png}}
    \vspace{.1cm}
    \caption{Cheshire (a) and its interrupt subsystem (b).}
    \label{fig:cheshire}
\end{figure}

\subsection{CVA6 extension}\label{subsec:arch:cva6}

We extend CVA6's interrupt handling logic to behave as follows when a \gls*{vm} is running: (i) if the incoming interrupt belongs to a higher privilege level, the core traps to that privilege level; (ii) if the incoming interrupt is directed to the currently running \gls*{vm} (i.e., the interrupt's and running \gls*{vm}'s \gls*{vsid} match), the interrupt is serviced by the running \gls*{vm}; (iii) if the incoming interrupt is directed to a different \gls*{vm}, the core traps to hypervisor mode if and only if the target \gls*{vm} has higher priority. Remarkably, item (iii) is crucial for the hypervisor to regain control of the core in case of high-priority events that must be handled by the dedicated \gls*{vm} with minimal latency.

% Furthermore, the {\vclic} extension introduces new \glspl*{csr} and extends the functionality of others. 
Furthermore, the virtualization extension requires the following \glspl*{csr} to be added: (i) \texttt{VSINTTHRESH}, the interrupt \emph{level} threshold (managing interrupt nesting in \gls*{clic}-based systems), (ii) \texttt{VSTVT}, the guest physical address of \gls*{vs} trap vector table (in \gls*{shv} mode), and (iii) \texttt{VSNXTI} for interrupt tail-chaining. In CLIC mode, the \texttt{vsie}, \texttt{vsip}, and \texttt{vsideleg} appear hardwired to zero, as their functionality is embedded in the \gls*{ic} itself. Finally, {\vclic} supports the original CLIC \gls*{shv} extension, allowing fine-grained management of virtual interrupts vectoring.

% removed citation from ~\cite{buttazzo2011hard, liu1973scheduling}


==> text/eval_2.tex <==
\section{Evaluation}
\label{sec:eval}
% We evaluate the performance of {\vclic} by measuring interrupt latency and jitter (as defined in~\cref{subsec:back:term}) in a virtualized environment and assessing the effects of micro-architectural state and resource contention on such metrics. 
% %
% Furthermore, we assess the area overhead of our solution compared to the baseline \gls*{clic}. Finally, we compare our results with those of related state-of-the-art solutions.

\subsection{Framework}\label{subsec:eval:frame}

%
To carry out fast and cycle-accurate latency measurements, we integrate {\vclic} into the Cheshire \gls*{soc} shown in~\cref{fig:cheshire} and emulate the system on a Digilent Genesys 2 FPGA board. On FPGA, Cheshire is configured with one CVA6 core and {\vclic} pair, 64 input interrupt lines, \SI{32}{\kibi\byte} of data and instruction cache, \SI{128}{\kibi\byte} of last-level cache, and is constrained to run at \SI{50}{\mega\hertz}. As a \gls*{sw} stack, we use two Hypervisors: the Bao \gls*{sph}~\cite{Martins2020BaoAL} and the Xvisor \gls*{dph}~\cite{XVISOR}, both open-source. 
Bao allows pinning a virtual guest to a physical core, improving the overall system determinism. We use it to assess the interrupt latency and jitter of {\vclic} in a built-in, predictable \gls*{sw} setting. Xvisor, in contrast, allows multiple \gls*{vm} guests to be assigned to a single physical core. We use Xvisor to assess interrupt prioritization and preemption across \gls*{vm} guests. 
% ({\vclic}'s \texttt{VSPRIO} extension). 
% We evaluate our implementation by comparing the interrupt latency of the FreeRTOS \gls*{rtos} with different \glspl*{ic}. To estimate the effect of resource contention in \glspl*{dph}, we run Linux and FreeRTOS on top of XVisor and measure the worst-case interrupt latency upon context-switch events. 

\subsection{Functional}\label{subsec:eval:func}

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.8\columnwidth]{example-image-b}
    % \includesvg[width=\columnwidth]{fig/performance.svg}
    \includegraphics[width=\columnwidth]{fig/interrupt_latency.pdf}
    % \includegraphics[width=\columnwidth]{fig/interrupt_latency_a.pdf}
    \caption{Interrupt latency comparison for \textit{bare-metal} (left), and \textit{virtualized} with FreeRTOS on top of Bao (right) scenarios. 
    }
    \label{fig:latency}
\end{figure}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=\columnwidth]{fig/latency_breakdown.pdf}
%     \includegraphics[width=\columnwidth]{fig/variability.pdf}
%     \caption{Interrupt latency breakdown and impact of caches and TLBs architectural state. CVA6 executes a bare-metal guest \gls*{vm} on top of the Bao \gls*{vmm}.}
%     \label{fig:latency_breakdown}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includesvg[width=\columnwidth]{fig/context_switch.svg}
%     \caption{Impact of {\vclic}'s \texttt{VSPRIO} extension. 
%     We show the \gls*{clic} context switching overhead with 64 interrupts per \gls*{vm}. We use Linux and FreeRTOS as guest \glspl*{vm} under XVisor. The target platform is Cheshire deployed on FPGA.
%     %We show that \glspl*{vm} interrupt prioritization can reduce the time to completion of a time-critical task when multiple guests are executing on the same physical resource.
%     }
%     \label{fig:contextsw}
% \end{figure}

\subsubsection{Interrupt latency}

Interrupt latency includes both \gls*{hw} and \gls*{sw} contributions. We include \gls*{sw} contributions affected by the core and \gls*{ic} design in the interrupt latency measurement to ensure a fair comparison. These are, for instance, the time to save the interrupt context and to identify the interrupt source.
% decode the interrupt (e.g., by reading an interrupt ID from a dedicated register).

Following this definition, we evaluate the interrupt latency of external interrupt sources with various interrupt subsystems: (i) vanilla \mbox{RISC-V} PLIC implementation~\cite{plic}; (ii) vanilla \mbox{RISC-V} CLIC implementation~\cite{clic}; (iii) vanilla AIA implementation, i.e. one A-PLIC and one \gls*{imsic}~\cite{costaopen}; and (iv) vCLIC proposed in this work. 
% Each subsystem is integrated into Cheshire and deployed on FPGA, as described in~\cref{subsec:eval:frame}. 

On the \gls*{sw} side, CVA6 executes in two settings: non-virtualized, or bare-metal, and virtualized, using FreeRTOS \gls*{vm} on top of the Bao monitor. We collect the interrupt latencies by running each experiment 100 times, assuming a warm micro-architectural state (i.e., we do not flush the caches and TLBs between iterations). This setup represents a lower bound on the expected interrupt latency, which can be affected by several factors, as discussed in the following sections.

\Cref{fig:latency} reports the best (minimum) and worst (maximum) interrupt latency of a single external interrupt source (e.g., a programmable timer) for each scenario. We observe a significant increase of about 20$\times$ in the interrupt latency of configurations (i) and (ii) without \gls*{hw}-assisted interrupt virtualization. The increase is due to the overhead of the \gls*{ic} \gls*{sw} emulation that the hypervisor must perform in the absence of \gls*{hw} support. The PLIC emulation results in a larger overhead due to the extra memory access required by the PLIC to read the interrupt ID that must be emulated by the hypervisor. Virtualization does not affect interrupt latency for both the \gls*{aia} and the {\vclic} configurations. The {\vclic} achieves a lower interrupt latency than \gls*{aia} due to the use of wired interrupts instead of interconnect-dependent \glspl*{msi}. 

\subsubsection{Interrupt jitter}

We identify two main contributions to the interrupt jitter: (i) instruction and data caches and (ii) TLBs. 
We assume two states for each component, i.e., \textit{warm} (recently accessed) and \textit{cold} (not recently accessed). We assess the impact of such components by measuring the interrupt latency of a custom bare-metal guest with virtual memory support under varying initial states of each element. On average, we observe that the interrupt latency --- independently from the \gls*{ic} --- is about 8$\times$ higher when caches are cold. As expected, cache misses only impact the \gls*{sw} contributions to the interrupt latency, such as the context save and restore and the interrupt decoding operations.  Conversely, TLB misses caused by cold TLBs result in a moderate \SI{5}{\percent} average slowdown. This happens because, for simple interrupt handlers, the entire \gls*{isr} fits within a single page.
% To enforce the reset of a component to a cold state, we use dedicated RISC-V instructions, i.e., \texttt{fence.i} \cite{RISCV_I} for the instruction cache and \texttt{sfence.vma} for the TLBs.

% To assess the impact of TLBs and cache hierarchy on interrupt latency, we use a custom bare-metal guest with virtual memory support and conduct measurements under varying initial states of each component, resulting in the four scenarios illustrated in \cref{fig:latency_breakdown}. The figure delineates a breakdown of the overall interrupt latency into six primary phases, from core interrupt acknowledgment to return to program execution. While the first four phases directly contribute to the interrupt latency, the remaining (context restore and return to program execution) contribute to the total interrupt handling time.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{fig/interrupt_latency.pdf}
%     % \caption{Interrupt latency comparison for \textit{non-virtualized}, or bare-metal (left-hand side), and \textit{virtualized}, running FreeRTOS \gls*{vm} on top of Bao (right-hand side). 
%     % % Each bar represents a different interrupt subsystem integrated in Cheshire and deployed on FPGA.
%     % }
%     \caption{Interrupt latency comparison for \textit{bare-metal} (left), and \textit{virtualized} with FreeRTOS on top of Bao (right) scenarios. 
%     % Each bar represents a different interrupt subsystem integrated in Cheshire and deployed on FPGA.
%     }
%     \label{fig:latency}
% \end{figure}

\subsection{System resources contention}\label{subsec:eval:contention}

% \Cref{subsec:eval:func} focuses on a single interrupt source targeting a \gls*{vm} running on top of a \gls*{sph}. We do not capture the worst-case interrupt latency by limiting the analysis to such a use case. \glspl*{mcs} typically have strict requirements for predictability and worst-case execution times to guarantee real-time performance and responsiveness to critical events. In this section, we discuss other possible scenarios that impact the worst-case interrupt latency.
To assess the worst-case interrupt latency, we expand our experiments to consider \gls*{hw} resource contention. We identify three main reasons for increased interrupt latency due to resource contention: (i) interrupt arbitration, (ii) bus contention, and (iii) \gls*{vm} interference.

\subsubsection{Interrupt arbitration}
% We refer to \textit{interrupt contention} as the scenario in which multiple interrupt requests are raised simultaneously. 
% Nearly every \gls*{ic} supports some interrupt prioritization. 
The {\vclic} prioritizes interrupts based on the assigned privilege mode, level, and priority, as well as based on a configurable \gls*{vm} priority (\texttt{VSPRIO} extension). However, this only affects the ordering of interrupts before they are serviced. Once an interrupt request is taken, higher-priority incoming interrupts may be delayed depending on the \gls*{ic} and \gls*{sw} implementation. {\vclic} minimizes the impact of interrupt contention through interrupt nesting~\cite{clic,CV32RT}, and extends this feature to virtual interrupts, allowing efficient implementations of preemptible \glspl*{isr}.

\subsubsection{Bus contention}
Existing virtualized systems are commonly based on \glspl*{msi}. \glspl*{msi} are mostly used in server-class computing systems, where predictability and real-time features are not critical requirements. As shown by Marques~et~al.~\cite{IEAIA_MINHO}, some system interconnect topologies can increase the average interrupt latency by up to 7$\times$ due to bus contention for \gls*{aia}-based systems, along with a significant rise (about \SI{750}{\nano\second} at \SI{50}{\mega\hertz}) in the response jitter over time. Unlike \gls*{msi}-based systems, we highlight that our proposed {\vclic} is entirely free from bus interference, regardless of the system interconnect topology, as it relies on core-local wired interrupt lines.

\subsubsection{Inter-\gls*{vm} interference}

In systems relying on \glspl*{dph}, interrupt latencies can vary substantially over time, depending on the resource allocation status at the time of the interrupt. To evaluate such scenarios, we run XVisor with Linux and FreeRTOS as guests. We evaluate the worst-case scenario -- a critical interrupt directed to FreeRTOS arrives while Linux is running -- by measuring the time required by the system to preempt the Linux execution in favor of FreeRTOS. On Cheshire, XVisor takes approximately $35000$ clock cycles to perform a \gls*{vm} context switch. As discussed in section \ref{subsubsec:arch:vsprio}, if the \texttt{VSPRIO} extension is disabled, the hypervisor must also save the configuration of interrupts delegated to the \gls*{vm} being switched out and set the configuration for the next \gls*{vm}. The performance degradation due to the additional interrupt context associated with each \gls*{vm} is proportional to the amount of interrupts delegated to the \gls*{vm}. The \gls*{clic} context switch requires up to $10000$ clock cycles for \glspl*{vm} with 64 virtual interrupts, increasing the overall context switch time by almost $30\%$.
Conversely, the context switch overhead is more tolerable if few interrupts are delegated to a \gls*{vm}, down to about $1250$ clock cycles in case of a single virtual interrupt per \gls*{vm}.

% If an interrupt directed to the safety-critical \gls*{rtos} becomes pending while another \gls*{vm} is scheduled, the incoming interrupt must wait for the hypervisor to resume the execution of the \gls*{rtos} before being serviced. In figure \ref{fig:contextsw}, we evaluate three possible scenarios in which an hypervisor can handle this, depending on the hardware support.

% A na\"ive implementation could mask the incoming interrupt until the target \gls*{vm} is scheduled, strongly impacting the worst-case interrupt latency. 
% A better approach leverages interrupt pre-emption mechanism based on an interrupt's target privilege mode. By dynamically configuring interrupts assigned to every inactive \glspl*{vm} to be delegated to \texttt{HS}-mode, privileged software can prioritize critical events, preempting non-critical \glspl*{vm} in favor of high-priority ones. As discussed in section \ref{subsubsec:arch:vsprio}, this approach incurs in the cost of increased context-switching time due to additional CLIC registers that must be saved and restored by the \gls*{vmm}.
% Finally, leveraging the \texttt{VSPRIO} extension, {\vclic}-based systems can reduce the worst-case interrupt latency by eliminating the need for reconfiguring the \gls*{clic} upon context-switch, thanks to hardware support for interrupt prioritization based on the target \gls*{vm}.

% The performance penalty for \gls*{clic} context-switches can be detrimental, especially when targeting \glspl*{mcs}. However, if only a few interrupts are delegated to a \gls*{vm}, the number of registers to be context-switched might not be high enough to justify the overhead of adding a per-interrupt extra configuration register. On our evaluation setup we measure a \gls*{vm} context-switching time of approximately 35000 clock cycles, when running Linux and FreeRTOS on top of XVisor. The \gls*{clic} context-switching takes between 1000 and 10000 clock cycles, depending on the amount of configuration registers to save / restore.

% ----------------------------------------------------------------------------

% I collected some numbers of a dummy CLIC context switch for a clic configuration with 64 interrupt lines. I run a few experiments that do the context switch of 1<=N<=64 interrupts, where N represents the amount of interrupt lines delegated to the VM being switched in / out. It takes between 1000 (N=1) and 10000 (N=64) cycles to do switch in + switch out of the configuration registers. It may not be the most optimized implementation but I think we can metion it as an extimate of the time we save by avoiding context switch.

% \todo{Work in progress to rewrite this better}

% --------------------------------------------------------------------------------
% Previous version:

% For systems managed by \glspl*{dph}, scenarios where a pending interrupt is directed to an inactive \gls*{vm} have to be considered especially for \glspl*{mcs}. In~\cref{fig:contextsw}, we illustrate this for a \gls*{mcs} running Linux alongside an \gls*{rtos} performing safety-critical tasks.

% A simple implementation might implicitly mask the incoming interrupt until the target \gls*{vm} is scheduled, which does not meet \gls*{mcs} requirements. A better approach leverages interrupt prioritization based on the target privilege mode. By configuring interrupts assigned to inactive \glspl*{vm} to be delegated to the hypervisor, privileged software can prioritize events, preempting non-critical \glspl*{vm} in favor of high-priority ones, at the cost of increased context switching time due to additional CLIC registers.

% The \texttt{VSPRIO} extension aims to reduce worst-case interrupt latency by eliminating the need for an extra \gls*{clic} context switching, thanks to hardware support for interrupt prioritization based on the target \gls*{vm}.

% There are mainly three other scenarions that can cause interrupt latencies to increase: (i) interrupt contention, (ii) bus contention, and (iii) VM contention. We refer to interrupt contention as the delay of a high priority interrupt due to a lower priority interrupt being serviced. This can happen both at the hardware and software levels. The CLIC \gls*{ic} minimizes the impact of interrupt contention by supporting interrupt nesting by means of interrupt levels~\cite{clic,CV32RT}. In MSI-based systems, bus contetion is another factor that can affect interrupt latency. Depending on the type of interconnect, MSI, which fundamentally are implemented as writes to specific memory mapped registers, can be affected by the amount of traffic on the bus. \todo{cite minho work for AIA interference?}. The vCLIC performance is not affected by bus contention, as it relies on wired interrupts instead of MSIs.
% Finally, we evaluate the worst case interrupt latency for dynamic partitioning virtualization, in which a guest operating system is not guaranteed to be executing at the time of receiving an interrupt. We assess the VM context switch time by running Linux and FreeeRTOS on top of Xvisor. Upon receiving an interrupt which is delegated to a inactive VM, the vCLIC can be configured to notify the hypervisor, which is then responsible to perform a VM context switch and to notify the interrupted VM. On Cheshire, we measure an average context-switch time of 35000 cycles, which is two order of magnitude higher than the static-partitioning use-case.

% \todo{TODO: complete with description of figure 7.}

\subsection{Implementation}\label{subsec:eval:impl}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.85\columnwidth]{fig/cheshire_area_breakdown_hbar.pdf}
%     \caption{Cheshire area breakdown, 64 wired input interrupts, synthesis in Intel16 FinFet. {\vclic} is instantiated with \texttt{VSPRIO} extension enabled and 1 priority bit (minimal configuration).}
%     \label{fig:cheshire-footprint}
% \end{figure}

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.5\columnwidth]{example-image-b}
    \includegraphics[width=0.9\columnwidth]{fig/vsclic_area_breakdown_hbar.pdf}
    \caption{\texttt{VSCLIC} area breakdown compared to vanilla CLIC. 
    }
    \label{fig:vsclic-footprint}
\end{figure}

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.5\columnwidth]{example-image-b}
    \includegraphics[width=0.9\columnwidth]{fig/vsprio_area_breakdown.pdf}
    \caption{\texttt{VSPRIO} area impact on {\vclic} with the number of priority bits. Case 0 indicates VSCLIC-only implementation.}
    \label{fig:vsprio-footprint}
\end{figure}

We synthesize {\vclic} as part of the Cheshire platform, as described in~\cref{subsec:eval:frame}. We use Synopsys Design Compiler 2022.03, targeting Intel 16 FinFet technology at \SI{1.1}{\giga\hertz}, SS corner, and \SI{125}{\celsius}.
One gate equivalent (GE) for this technology equals \SI{0.233}{\micro\meter\squared}.
Our extension does not affect the critical path of the design.

\Cref{fig:vsclic-footprint} shows the area overhead introduced by the \texttt{VSCLIC} extension compared to vanilla \gls*{clic}, totaling about \SI{8}{\kilo\GE}. Most of the additional resources are due to the increased memory-mapped registers. \gls*{clic}'s binary tree size to propagate the highest level and priority interrupt is equally affected with roughly \SI{27}{\percent} increase. We evaluate the impact of the \texttt{VSPRIO} extension based on the number of priority levels, as shown in~\cref{fig:vsprio-footprint}. The arbitration tree size grows almost linearly with the number of implemented priority bits. 
% We observe that, albeit conducting a detailed space exploration of area variation, a realistic number of priority bits lies in the range 2-4, meaning 4 to 16 priority levels.

Finally, we complete the in-system assessment by measuring the area of Cheshire and the relative impact of {\vclic}. Accounting for the memory macros footprint, {\vclic} occupies merely \SI{1}{\percent} of the system.
Compared to platform-wide centralized approaches, this result justifies a per-core, distributed solution for interrupt management in a virtualized scenario.


